Elliptic Feynman integrals and pure functions

We propose a variant of elliptic multiple polylogarithms that have at most logarithmic singularities in all variables and satisfy a differential equation without homogeneous term. We investigate several non-trivial elliptic two-loop Feynman integrals with up to three external legs and express them in terms of our functions. We observe that in all cases they evaluate to pure combinations of elliptic multiple polylogarithms of uniform weight. This is the first time that a notion of uniform weight is observed in the context of Feynman integrals that evaluate to elliptic polylogarithms.

==> pure_empls_2.tex <==
% !TEX root = pure_paper.tex

\section{Elliptic polylogarithms and pure functions}
\label{sec:pure_empls}

In the previous sections we have reviewed multiple polylogarithms, both ordinary and elliptic. We have seen that the elliptic and non-elliptic cases share many properties. In this section we argue how the concept of pure functions can be extended from ordinary to elliptic MPLs. Before we present the definition of pure eMPLs, we present in the next subsection the motivation for that definition. 

\subsection{Motivation}
A priori, it is not entirely clear how to extend the definition of pure functions to the elliptic case. Thus we can only proceed by example and analyse available results for Feynman integrals that evaluate to eMPLs. 
A naive definition of a pure elliptic Feynman integral could consist in considering $\mathbb{Q}$-linear combinations of elliptic polylogarithms $\textrm{E}_4$ of the same length or weight. Such a naive definition, however, soon reaches its limits, as we now demonstrate. 

In ref.~\cite{Broedel:2017siw} the two-loop sunrise integral in $D=2-2\eps$ with three equal masses was computed in terms of the eMPLs $\textrm{E}_4$. More precisely, consider the family of integrals
\beq
S_{n_1n_2n_3}(p^2,m^2) = -\frac{e^{2\gamma_E\eps}}{\pi^D}\int\frac{d^Dk\,d^Dl}{(k^2-m^2)^{n_1}(l^2-m^2)^{n_2}((k+l+p)^2-m^2)^{n_3}}\,,
\eeq
with $n_i\in \mathbb{N}$.
Using IBP identities, every integral in the family can be written as a linear combination of the following three master integrals,
\beq\bsp\label{eq:sunrise_masters}
S_0(p^2,m^2)&\, = S_{110}(p^2,m^2)\,,\\
 S_1(p^2,m^2) &\,= S_{111}(p^2,m^2)\,,\\
  S_2(p^2,m^2)&\, = S_{112}(p^2,m^2)\,.
\esp\eeq
$S_0$ is the product of two one-loop tadpole integrals and will not be discussed any further. For now, we focus only on the master integral $S_1$, and we return to $S_2$ in Section~\ref{sec:applications}.
The result for $S_1$ reads~\cite{Broedel:2017siw}
\beq\bsp
\label{eqn:S111_result}
S_{1}(p^2,m^2) 
&\,=\frac{1}{(m^2+p^2)c_4}\Biggr[\frac{1}{c_4}\Efe{0&0}{0&0}{1}{\vec a}-2\Efe{0&-1}{0&\infty}{1}{\vec a}-\Efe{0&-1}{0&0}{1}{\vec a}\\
&\,\phantom{=\frac{1}{(m^2+p^2)c_4}\Biggr[}-\Efe{0&-1}{0&1}{1}{\vec a}-\Efe{0&1}{0&0}{1}{\vec a}\Biggr] + \ord(\eps)\,,
\esp\eeq
where the vector of branch points $\vec a$ is
\begin{equation}\begin{split}
  \label{eqn:roots}
\vec a = \left(\frac{1}{2}(1+\sqrt{1+\rho}),\frac{1}{2}(1+\sqrt{1+\overline{\rho}}),\frac{1}{2}(1-\sqrt{1+\rho}),\frac{1}{2}(1-\sqrt{1+\overline{\rho}})\right)\,.
\end{split}\end{equation}
with
\begin{equation}
    \rho = -\frac{4m^2}{(m+\sqrt{-p^2})^2} \textrm{~~and~~} \overline{\rho} = -\frac{4m^2}{(m-\sqrt{-p^2})^2}\,. 
\end{equation}
The result for $S_{1}$ in eq.~\eqref{eqn:S111_result} is not pure (not even up to an overall algebraic factor), because not all the $\textrm{E}_4$ functions are multiplied by rational \emph{numbers}, but the first term in square brackets is multiplied by the algebraic function $1/c_4$. There are, however, strong motivations to believe that the two-loop sunrise integral should define a pure function of some sort: First, the corresponding result in the case of three different masses can be written as a $\mathbb{Q}$-linear combination of $\textrm{E}_4$ functions, and no additional algebraic prefactor is needed~\cite{Broedel:2017siw}. Second, in the case where at least one propagator is massless, the integral can be evaluated in terms of pure linear combination of ordinary MPLs. Third, the equal-mass sunrise integral $S_{1}(p^2,m^2)$ can also be written in terms of iterated integrals of Eisenstein series~\cite{Adams:2017ejb,Broedel:2018iwv}, and also in this representation no additional algebraic prefactor is needed. 

Based on this example, we see that a naive definition of `elliptic purity' via the basis of eMPLs $\textrm{E}_4$ does not have the desired properties. Instead of working with the basis of $\textrm{E}_4$ functions, we can change basis and consider the basis of eMPLs $\widetilde{\Gamma}$ on the complex torus. We observe that when expressed in terms of this basis, the equal-mass sunrise integral is a $\mathbb{Q}$-linear combination of $\widetilde{\Gamma}$ functions (up to an overall factor), i.e., it is a function that can be qualified as pure. The final expression for $S_{1}$ in terms of pure functions will be given in Section~\ref{sec:applications}. We therefore propose that the functions $\widetilde{\Gamma}$ are pure functions, and a Feynman integral is pure if it can be expressed as a $\mathbb{Q}$-linear combination of such functions (up to overall normalisation). As a motivation for this proposal, we point out that, just like ordinary MPLs, the functions $\widetilde{\Gamma}$ have at most logarithmic singularities. Indeed, we have seen in Section~\ref{sec:empls} that the integration kernels $g^{(n)}(z,\tau)$ have at most simple poles, and so the one-forms $\omega_{ij}^{(n)}$ that appear in the total differential of $\gamtt{n_1 &\ldots& n_k}{z_1 & \ldots & z_k}{z}{\tau}$ have at most logarithmic singularities (see eqs.~\eqref{eq:gamma_differential} and~\eqref{eq:empl_letter}). Hence, seen as a function in many variables, $\gamtt{n_1 &\ldots& n_k}{z_1 & \ldots & z_k}{z}{\tau}$ has only logarithmic singularities in each variable, but no poles (because the differential of a pole is a pole of order at least two). This property is identical to the corresponding property for ordinary MPLs, as can easily be seen from the fact that the total differential of an ordinary MPL in eq.~\eqref{eq:MPL_tot_diff} only involves logarithmic one-forms. The $\textrm{E}_4$, instead, do not only have logarithmic singularities, but also poles when seen as a function of many variables. Indeed, consider the function $\Efe{-1}{c}{x}{\vec a}$, with $c\neq\infty$. Using eqs.~\eqref{eq:psi_to_g} and~\eqref{eq:Z4_to_g1} (and assuming for simplicity that $z_0=0$), we find
\begin{align}
\nonumber\Efe{-1}{c}{x}{\vec a} &\,= \gamtt{1}{z_c}{z_x}{\tau} - \gamtt{1}{-z_c}{z_x}{\tau} + \left[g^{(1)}(z_c-z_{\ast},\tau) + g^{(1)}(z_c+z_{\ast},\tau)\right]\,\gamtt{0}{0}{z_x}{\tau}\\
&\,=\gamtt{1}{z_c}{z_x}{\tau} - \gamtt{1}{-z_c}{z_x}{\tau} -\omega_1\,Z_4(c,\vec a) \,\gamtt{0}{0}{z_x}{\tau}\,.
\end{align}
While the functions $\widetilde{\Gamma}$ have at most logarithmic singularities, the function $Z_4(c,\vec a)$ has a pole at $c=\infty$. Hence, we see that unlike the $\widetilde{\Gamma}$ functions, the $\textrm{E}_4$ functions have poles (we stress, however, that in the variable $x$ they only have logarithmic singularities, because the kernels $\psi_n(c,x,\vec a)$ have at most simple poles in $x$). Based on these considerations we propose the following definition of \emph{pure functions}:
\begin{quote}
\emph{A function is called pure if it is unipotent and its total differential involves only pure functions and one-forms with at most logarithmic singularities.}
\end{quote}
Sums and product of pure functions are obviously pure. Finally, we postulate that a pure function remains pure under specialisation of the arguments. This allows us in particular to extend the definition from function to numbers.


While the functions $\widetilde{\Gamma}$ provide a basis of pure eMPLs, this basis is often not the most convenient one when working with Feynman integrals:
\begin{enumerate}
\item Feynman integrals often have an intrinsic notion of `parity', defined in the following way: Although the final analytic result for a Feynman integral may involve square roots, the original integrand is a purely rational object. Hence, the final analytic result including square roots must be independent of the choice of the branch of the root. This implies that the pure function part must have definite `parity' with respect to the operation of changing the sign of the root.  For example, we see that the one-loop bubble integral in eq.~\eqref{eq:one-loop} is independent of the sign of the square root, and both the algebraic prefactor and the pure function part are odd functions. In the case of eMPLs, changing the sign of the square root corresponds to the operation $(x,y) \leftrightarrow (x,-y)$. Since $(x,y) = (\kappa(z,\vec a),c_4\,\kappa'(z,\vec a))$, this operation corresponds on the torus to changing the sign of $z$. We would thus like to have a basis of pure functions that have definite parity under this operation. The basis $\widetilde{\Gamma}$ does not have this property, and we prefer to work with the alternative basis that makes this symmetry manifest.
\item From the mathematical point of view, elliptic curves and the functions associated to them are most naturally studied in terms of complex tori and the coordinate $z$. Feynman integrals, however, are more naturally expressed in terms of the variables $(x,y)$, because these variables are more directly related to the kinematics of the process under consideration. We would therefore like to have a basis of pure eMPLs formulated directly in terms of the variables $(x,y)$.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Pure elliptic multiple polylogarithms}
In this section we introduce a new class of iterated integrals on the elliptic curve defined by the polynomial equation $y^2=P_4(x)$ with the following properties:
\begin{enumerate}
\item They form a basis for the space of all eMPLs.
\item They are pure.
\item They have definite parity.
\item They manifestly contain ordinary MPLs as a special case.
\end{enumerate}
The definition reads
\beq\label{eq:cE4_def}
\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}} = \int_0^xdt\,\Psi_{n_1}(c_1,t,\vec a)\,\cEf{n_2 & \ldots & n_k}{c_2 & \ldots& c_k}{t}{\vec a}\,,
\eeq
with $n_i\in\mathbb{Z}$ and $c_i\in\widehat{\mathbb{C}}$. The length and the weight are specified in analogy with the case of the $\textrm{E}_4$ functions in eq.~\eqref{eq:E4_def}. The integration kernels are defined implicitly through the identity (for $n\ge 0$)
\begin{align}\label{eq:Psi_to_gh}
dx\,&\Psi_{\pm n}(c,x,\vec a)\\
\nonumber& = dz_x\,\left[g^{(n)}(z_x-z_c,\tau)  \pm g^{(n)}(z_x+z_c,\tau) - \delta_{\pm n,1}\,\left(g^{(1)}(z_x-z_\ast,\tau) + g^{(1)}(z_x+z_\ast,\tau)\right)\right]\,.
\end{align}
It is easy to check that the class of functions defined in this way satisfies the three properties outlined above: First, there is a one-to-one map between the kernels $\Psi_{\pm n}$ and the functions $g^{(n)}(z_x\pm z_c,\tau)$. Since the latter define the basis of eMPLs $\widetilde{\Gamma}$, there is a one-to-one map between the functions $\cE_4$ and $\widetilde{\Gamma}$, and so the iterated integrals in eq.~\eqref{eq:cE4_def} define a basis for the space of all eMPLs. Second, since the coefficients in eq.~\eqref{eq:Psi_to_gh} are all $\pm1$, the functions $\cE_4$ can be written as a $\mathbb{Q}$-linear combination of $\widetilde{\Gamma}$ functions, and so the $\cE_4$ functions are pure. Finally, it is easy to see that eq.~\eqref{eq:Psi_to_gh} has definite parity under changing the sign of $z_x$. Hence, the $\cE_4$ functions define a pure basis of eMPLs with definite parity. The term proportional to a Kronecker $\delta$ is conventional, and added so that (cf. eq.~\eqref{eq:psi_to_g})
\beq
dx\,\Psi_1(c,x,\vec a) = \frac{dx}{x-c}\,,\qquad c\neq \infty\,.
\eeq
In this way we make manifest that ordinary MPLs are a subset of eMPLs,
\beq\label{eq:cE4_to_G}
\cEf{1 & \ldots & 1}{c_1 & \ldots& c_k}{x}{\vec{a}} = G(c_1,\ldots,c_k;x)\,,\qquad c_i\neq \infty\,.
\eeq
Given the properties that the iterated integrals in eq.~\eqref{eq:cE4_def} fulfil, we argue that this class of functions is very well suited to express Feynman integrals that can be written in terms of eMPLs. We will illustrate this on several non-trivial elliptic Feynman integrals with up to four external legs in Section~\ref{sec:applications}. In the remainder of this section we study in more detail the properties of the $\cE_4$ functions.

So far we have only defined the kernels $\Psi_{\pm n}$ in eq.~\eqref{eq:Psi_to_gh} implicitly through their relationship to the coefficients of the Eisenstein-Kronecker series. In ref.~\cite{Broedel:2017kkb} it was shown that there is a one-to-one map between the $g^{(n)}$ functions and the kernels $\psi_{\pm n}$ defined in Section~\ref{sec:empls}. Using the result of ref.~\cite{Broedel:2017kkb} we can thus give an explicit representation of the kernels that appear in eq.~\eqref{eq:cE4_def}. We present here explicitly the formul\ae\ up to $n=1$. The extension to higher values of $n$ is straightforward. For $n=0$, we find
\beq\label{eq:pure_psi0}
\Psi_0(0,x,\vec a) = \frac{1}{\omega_1}\,\psi_0(0,x,\vec a)= \frac{c_4}{\omega_1\,y}\,.
\eeq
For $n=1$, we have (with $c\neq \infty$)
\begin{align}
\nonumber \Psi_1(c,x,\vec a) &\,= \psi_1(c,x,\vec a)= \frac{1}{x-c}\,, \\
\label{eq:pure_psi1}\Psi_{-1}(c,x,\vec a) &\,= \psi_{-1}(c,x,\vec a) + Z_4(c,\vec a)\,\psi_0(0,x,\vec a) = \frac{y_c}{y(x-c)} + Z_4(c,\vec a)\,\frac{c_4}{y}\,,\\
\nonumber\Psi_{1}(\infty,x,\vec a) &\,= -\psi_{1}(\infty,x,\vec a) = -Z_4(x,\vec a)\,\frac{c_4}{y}\,,\\
\nonumber\Psi_{-1}(\infty,x,\vec a) &\,= \psi_{-1}(\infty,x,\vec a) - \left[\frac{a_1}{c_4}+ 2 G_{\infty}(\vec a)\right]\,\psi_0(0,x,\vec a) = \frac{x}{y}   -\frac{1}{y} \left[{a_1}+ 2c_4\, G_{\infty}(\vec a)\right]\,.
\end{align}
The quantity $G_{\infty}(\vec a)$ in the last equation corresponds to the image of $z_\ast$ under the function $g^{(1)}$. It can be explicitly given in terms of incomplete elliptic integrals of the first and second kinds,
\beq\bsp\label{eq:G_infty_def}
G_{\infty}(\vec a) &\,\equiv \frac{1}{\omega_1}\,g^{(1)}(z_{\ast},\tau)=\lim_{x\to\infty}\left[\frac{y}{2c_4\,(x-a_1)} - \frac{1}{2}\,Z_4(x,\vec a)\right]\\
&\,=i\,\textrm{E}(\sqrt{\alpha}|1-\lambda)-i\,\textrm{F}(\sqrt{\alpha}|1-\lambda)\,\left[\frac{1+\lambda}{3}-2\,\frac{\eta_1}{\omega_1}\right] - \frac{a_{14}}{2c_4}\,,
\esp\eeq
where $\alpha$ and $\textrm{F}$ are given in eqs.~\eqref{eq:zstar} and~\eqref{eq:F_def}, and $\textrm{E}$ denotes the incomplete elliptic integral of the second kind,
\beq\label{eq:E_def}
\textrm{E}(x|\lambda) = \int_0^x{dt}{\sqrt{\frac{1-\lambda t^2}{1-t^2}}}\,.
\eeq 
\claudecomment{Shall we also give $n=2$? Maybe in an appendix, because the results are a bit more lengthy.}
We see that the price to pay to have integration kernels that define pure functions is that the kernels involve the functions $Z_4$ and $G_{\infty}$. While in general these functions are transcendental, in applications these functions often simplify and can be expressed in terms of algebraic functions, thereby simplifying greatly the analytic structure of the integration kernels $\Psi_n$. 

Let us look at the case of $G_{\infty}$. There is one case where a closed analytic formula for it can be
derived which does not involve transcendental functions. In particular, let us go back to the formula for $z_*$, 
eq.~\eqref{eq:zstar}, which we report here for convenience
$$
z_* = -i\, \frac{{\rm F}(\sqrt{\alpha}| 1-\lambda)}{2 {\rm K}(\lambda)}\,.
$$
Let us imagine, as it often happens in physics applications, that $z_*$ were a function of $\tau$ only, namely
$$z_* = a + b\, \tau\,,$$
 where $\tau$ is as usual the ratio of the two periods $\tau = \omega_2/\omega_1$. 
 Clearly, since the two periods
 are only function of $\lambda$, this implies that in eq.~\eqref{eq:zstar} $\alpha$ and $\lambda$ cannot be independent,
 but instead $\alpha=\alpha(\lambda)$\,. Now, equating the two expressions for $z_*$ we can write
 \begin{equation}
 a + b\, \tau = -i\, \frac{{\rm F}(\sqrt{\alpha}| 1-\lambda)}{2 {\rm K}(\lambda)}\,, \label{eq:1}
 \end{equation}
and differentiating on both sides with respect to $\lambda$ we obtain
 \begin{align}
 b\, \frac{d \tau}{d \lambda} &= -i\, \frac{d}{d\lambda}\frac{{\rm F}(\sqrt{\alpha}| 1-\lambda)}{2 {\rm K}(\lambda)}\,. \label{eq:2}
 \end{align}
As it is well known, the derivative of ${\rm F}(\sqrt{\alpha}| 1-\lambda)$ involves the function ${\rm E}(\sqrt{\alpha}| 1-\lambda)$,
such that, by working out the derivative, we can invert eqs.~(\ref{eq:1},\ref{eq:2}) and express ${\rm F}(\sqrt{\alpha}| 1-\lambda)$
and ${\rm E}(\sqrt{\alpha}| 1-\lambda)$ in terms of $\tau$ and its derivative. Substituting these results into
eq.~\eqref{eq:G_infty_def}, we are then left with


\begin{align}
G_{\infty}(\vec a) &= -\frac{i \lambda  (\lambda -1) \alpha '(\lambda )}{\sqrt{(1-\alpha ) \alpha } \sqrt{\alpha  (\lambda -1)+1}}
-\frac{i \sqrt{(1-\alpha ) \alpha }
   (\lambda -1)}{\sqrt{\alpha  (\lambda -1)+1}}-2 \,b\, \lambda  (\lambda -1) \omega _1 \tau '(\lambda )
   -\frac{a_{14}}{2 c_4}\,,
\end{align}
where $'$ indicates the derivative w.r.t. $\lambda$.
It is very easy to compute $\tau'(\lambda)$ as
\begin{align}
\tau'(\lambda) &= \frac{d}{d\lambda} \left(\frac{\omega_2}{\omega_1}\right) = \frac{i \pi }{(\lambda -1) \lambda  \, \omega_1^2}
\end{align}
such that the expression above becomes
\begin{align}
G_{\infty}(\vec a) &= -\frac{i \lambda  (\lambda -1) \alpha '(\lambda )}{\sqrt{(1-\alpha ) \alpha } \sqrt{\alpha  (\lambda -1)+1}}
-\frac{i \sqrt{(1-\alpha ) \alpha }
   (\lambda -1)}{\sqrt{\alpha  (\lambda -1)+1}} - b\,  \frac{2 \pi i }{  \, \omega_1}
   -\frac{a_{14}}{2 c_4}\,. \label{eq:G_start_algebraic}
\end{align}
Once the exact relation between $\alpha$ and $\lambda$ is known (which of course depends on the problem considered), eq.~\eqref{eq:G_start_algebraic} becomes explicit and can be used to derive the expression for $G_\infty$. We will see 
some explicit examples of this procedure below, when we present results for some Feynman integrals that evaluate
to elliptic polylogarithms.


We conclude this section by mentioning that $\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}$ may diverge whenever $c_k=0$, and we need to regularise the integral. This is a technical aspect which does not add anything conceptually new to the discussion. The reader interested in the details may refer to Appendix~\ref{app:regularisation}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Properties of pure eMPLs}
Before we discuss examples of Feynman integrals that can be expressed in terms of the pure basis of eMPLs defined in the previous subsection, we summarise here some of their properties. Most of these properties are inherited from the corresponding properties of the $\textrm{E}_4$ and $\widetilde{\Gamma}$ functions, but we collect them here for completeness.

\paragraph{Shuffle algebra.} Just like ordinary MPLs (and iterated integral in general), the $\cE_4$ functions form a shuffle algebra,
\beq\label{eq:shuffle_cE4}
\cE_4(A_1 \cdots A_k;x,\vec a)\,\cE_4(A_{k+1}\cdots A_{k+l};x,\vec a) = \sum_{\sigma\in \Sigma(k,l)}\cE_4(A_{\sigma(1)} \cdots A_{\sigma(k+l)};x,\vec a)\,,
\eeq
with $A_i=\left(\begin{smallmatrix}n_i\\ c_i\end{smallmatrix}\right)$.

\paragraph{Rescaling of arguments.} Just like ordinary MPLs, the $\cE_4$ functions are invariant under a simultaneous rescaling of the arguments (cf. eq.~\eqref{eq:rescaling}),
\beq
\cEf{n_1 & \ldots & n_k}{p\,c_1 & \ldots& p\,c_k}{p\,x}{p\,\vec{a}} = \cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}\,,\qquad p,c_k\neq 0\,.
\eeq

\paragraph{Unipotency, symbols and coaction.} The $\cE_4$ functions are pure linear combinations of $\widetilde{\Gamma}$ functions. The latter are unipotent~\cite{BrownLevin,Broedel:2018iwv}, i.e., they satisfy a differential equation without homogeneous term (cf. eq.~\eqref{eq:gamma_differential}). It immediately follows that the $\cE_4$ functions are also unipotent. We can then apply the construction of ref.~\cite{Brown:coaction} and define a notion of symbols and a coaction on $\cE_4$ functions, similar to the coaction on the $\widetilde{\Gamma}$ functions introduced in ref.~\cite{Broedel:2018iwv}.
For example, we have
\begin{align}
\nonumber\Delta&\left(\cEf{0&-1}{0&c}{x}{\vec{a}}\right) = \cEf{0&-1}{0&c}{x}{\vec{a}}\otimes 1 - \cEf{-1}{\infty}{x}{\vec{a}}\otimes \left[dz_c\right] + \cEf{-1}{c}{x}{\vec{a}}\otimes \left[dz_x\right]\\
& - \cEf{1}{c}{x}{\vec{a}}\otimes \left[dz_c\right] + \cEf{-2}{\infty}{x}{\vec{a}}\otimes \left[\frac{d\tau}{2\pi i}\right] - \cEf{0}{0}{x}{\vec{a}}\otimes \left[\omega^{(1)}(z_0-z_c,\tau)\right]\\
\nonumber&+\cEf{0}{0}{x}{\vec{a}}\otimes \left[\omega^{(1)}(-z_c,\tau)\right] + \cEf{0}{0}{x}{\vec{a}}\otimes \left[\omega^{(1)}(z_c,\tau)\right] \\
\nonumber&+\cEf{0}{0}{x}{\vec{a}}\otimes \left[\omega^{(1)}(z_c+z_0,\tau)\right]
+1\otimes S\,,
\end{align}
where $S$ denotes the symbol of $\cEf{0&-1}{0&c}{x}{\vec{a}}$,
\begin{align}
\nonumber&S = \big[dz_0 - dz_x\big|\omega ^{(1)}\left(z_0-z_c,\tau \right)\big] +\big[ dz_x-dz_0\big|\omega ^{(1)}\left(-z_c,\tau \right)\big] +\big[dz_0 - dz_x\big|\omega ^{(1)}\left(z_c,\tau \right)\big]\\
\nonumber& +\big[ dz_x -dz_0\big|\omega ^{(1)}\left(z_c+z_0,\tau \right)\big] +\big[ \omega ^{(1)}\left(z_0-z_c,\tau \right)\big|dz_0-dz_x\big] +\big[ \omega ^{(1)}\left(z_c+z_0,\tau \right)\big|dz_x+dz_c\big]\\
\nonumber& +\big[ \omega ^{(1)}\left(z_x-z_c,\tau \right)\big|dz_x-dz_c\big] -\big[ \omega ^{(1)}\left(z_c+z_x,\tau \right)\big|dz_c-dz_x\big] +\big[ \omega ^{(2)}\left(z_x-z_c,\tau \right)\big|\frac{d\tau}{2\pi i}\big] \\
&-\big[ \omega ^{(2)}\left(z_c+z_x,\tau \right)\big|\frac{d\tau}{2\pi i}\big] -\big[ \omega ^{(2)}\left(z_0-z_c,\tau \right)\big|\frac{d\tau}{2\pi i}\big] +\big[ \omega ^{(2)}\left(z_c+z_0,\tau \right)\big|\frac{d\tau}{2\pi i}\big]\,.
\end{align}
Note that via eq.~\eqref{eq:cE4_to_G} we can interpret every ordinary MPL as an eMPL. Very importantly, the definition of the symbol in the elliptic case agrees with the definition of the symbol of ordinary MPLs~\cite{ChenSymbol,Goncharov:2009tja,Brown:2009qja,Goncharov:2010jf,Duhr:2011zq}.

\paragraph{Closure under integration.} Consider the algebra $\cA_4$ generated by functions of the form
\beq
R(x,y) \, Z_4(x,\vec a)^m\,\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}\,,
\eeq
where $m\in\mathbb{N}$ and $R(x,y)$ is a rational function, with $y^2=P_4(x)$ and we assume that $\vec a$ and the $c_i$ are independent of $x$. Then every element of $\cA_4$ has a primitive with respect to $x$. This follows immediately from the corresponding statement with $\cE_4$ replaced by $\textrm{E}_4$, which was proved in ref.~\cite{Broedel:2017kkb} (see also ref.~\cite{BrownLevin}). The computation of the primitive is algorithmic, and can be done using the techniques of ref.~\cite{Broedel:2017kkb}.

\paragraph{Value at the infinite cusp.} For $\tau\to i\infty$, $\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}$ always reduces to a pure  combination of ordinary MPLs of weight $\sum_in_i$. This follows immediately from analysing how the coefficients of the Eisenstein-Kronecker series behave as $\tau\to i\infty$. In particular, they admit the Fourier expansions~\cite{Broedel:2014vla,Broedel:2015hia,Broedel:2017jdo}
\beq\bsp\label{eq:g_q_exp}
g^{(1)}(z,\tau) &= \pi  \cot(\pi z) + 4\pi \sum_{m=1}^{\infty}  \sin(2\pi m z) \sum_{n=1}^{\infty} q^{mn}\,,\\
g^{(k)}(z,\tau) \Big|_{k=2,4,\ldots} &=  - 2\zeta_k - 2 \frac{ (2\pi i)^k }{(k-1)!} \sum_{m=1}^{\infty}  \cos(2\pi m z) \sum_{n=1}^{\infty}n^{k-1} q^{mn} \,, \\
%
g^{(k)}(z,\tau) \Big|_{k=3,5,\ldots}&= - 2i \frac{ (2\pi i)^k }{(k-1)!} \sum_{m=1}^{\infty}  \sin(2\pi m z) \sum_{n=1}^{\infty}n^{k-1} q^{mn}\,,
\esp\eeq
with $q = \exp(2\pi i\tau)$.


\paragraph{Relationship to iterated integrals of Eisenstein series.} In ref.~\cite{Broedel:2018iwv} it was shown that whenever the arguments of $\gamtt{n_1 &\ldots& n_k}{z_1 & \ldots & z_k}{z_{k+1}}{\tau}$ are rational points\footnote{In the mathematics literature, these points are known as \emph{torsion points} of the elliptic curve.} of the form $z_i = \frac{r_i}{N} + \tau\frac{s_i}{N}$, $r_i,s_i,N\in\mathbb{Z}$ and $N>0$, then it can be expressed in terms of iterated integrals of Eisenstein series for $\Gamma(N) = \left\{\gamma\in SL(2,\mathbb{Z}):\gamma = \left(\begin{smallmatrix}1&0\\0&1\end{smallmatrix}\right)\!\!\mod N\right\}$. A spanning set for Eisenstein series for $\Gamma(N)$ is given by~\cite{Broedel:2018iwv,ZagierBonn}
\beq
h^{(n)}_{N,r,s}(\tau) =-\!\!\!\!\!\!\!\sum_{\substack{(\alpha,\beta)\in \mathbb{Z}^2\\ (\alpha,\beta)\neq(0,0)}}\frac{e^{2\pi i(s\alpha-r\beta)/N}}{(\alpha+\beta\tau)^{2n}}\,.
\eeq
The iterated integrals one needs to consider are thus
\beq\bsp\label{eq:I_Eisenstein_def}
I\left(\begin{smallmatrix} n_1& N_1\\ r_1& s_1\end{smallmatrix}\big|\ldots\big|\begin{smallmatrix} n_k& N_k\\ r_k& s_k\end{smallmatrix};\tau\right) = \int_{i\infty}^{\tau}d\tau'\,h_{N_1,r_1,s_1}^{(n_1)}(\tau')\,I\left(\begin{smallmatrix} n_2& N_2\\ r_2& s_2\end{smallmatrix}\big|\ldots\big|\begin{smallmatrix} n_k& N_k\\ r_k& s_k\end{smallmatrix};\tau'\right)\,,
\esp\eeq
By convention, we set $h_{0,0,0}^{(0)}(\tau)\equiv 1$. In general, these integrals require regularisation~\cite{Brown:mmv}. The weight of $I\left(\begin{smallmatrix} n_1& N_1\\ r_1& s_1\end{smallmatrix}\big|\ldots\big|\begin{smallmatrix} n_k& N_k\\ r_k& s_k\end{smallmatrix};\tau\right) $ is defined as $\sum_in_i$. Since every $\cE_4$ function can be written as a pure linear combination of $\widetilde{\Gamma}$'s, we conclude that a similar statement holds for $\cE_4$ functions. More precisely, consider the function $\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}$. If all of the arguments, as well as the point at infinity and the base point are mapped to rational points on the torus by Abel's map (i.e., $z_0$, $z_{\ast}$, $z_x$ and all of the $z_{c_i}$ are rational points), then we can express $\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}$ as a pure linear combination of uniform weight $\sum_i|n_i|$ of the iterated integrals defined in eq.~\eqref{eq:I_Eisenstein_def}.


\paragraph{Regularisation.} In the case where $(n_k,c_k) = (\pm1,0)$ the integral in eq.~\eqref{eq:cE4_def} is divergent and requires regularisation. This situation is similar to the case of ordinary MPLs, where the naive iterated integral representation for $G(0,\ldots,0;x)$ would be divergent, and instead one gives a special definition for the special case, cf.~\eqref{eq:GLog}. In the case of eMPLs, we have a divergence whenever $(n_k,c_k) = (\pm1,0)$, and so we need to give a special definition for the cases $\cEf{n_1 & \ldots & n_k}{0&\ldots&0}{x}{\vec a}$, with $n_i=\pm1$. We define, for $A_i=\left(\begin{smallmatrix}\pm1\\0\end{smallmatrix}\right)$,
\begin{align}\label{eq:eMPL_reg}
\cE_4(A_1\ldots A_k;x;\vec a) = \frac{1}{k!}\log^kx + &\sum_{l=0}^k\sum_{m=1}^l\sum_{\sigma}\frac{(-1)^{l+m}}{(k-l)!}\log^{k-l}x\\
\nonumber&\times\cE_4^{\textrm{R}}\left(A^{(m)}_{\sigma(1)}\ldots A^{(m)}_{\sigma(m-1)} A^{(m)}_{\sigma(m+1)}\ldots A^{(m)}_{\sigma(l)}\Big|A_m;x;\vec a\right)\,,
\end{align}
where the third sum runs over all shuffle $\sigma\in\Sigma(m-1,l-m)$ and $A_i^{(m)} = A_i$ if $i<m$ and $A_i^{(m)} = \left(\begin{smallmatrix}1\\0\end{smallmatrix}\right)$ otherwise. The $\cE_4^{\textrm{R}}$ are iterated integrals with suitable subtractions to render the integrations finite,
\beq
\!\!\!\cE_4^{\textrm{R}}\left(\begin{smallmatrix} n_1&\ldots & n_k \\ 0 &\ldots &0\end{smallmatrix}|\begin{smallmatrix} n_a \\ 0 \end{smallmatrix};x;\vec a\right) 
= \int_0^xdt_1\Psi_{n_1}(0,t_1)\int_{0}^{t_1}\ldots \int_{0}^{t_{k-1}}dt_k\left(\Psi_{n_a}(0,t_k) - \Psi_{1}(0,t_k)\right)\,.
\eeq
For example, we have
\beq
\cEf{-1}{0}{x}{\vec a} = \log x + \int_0^xdt\left(\Psi_{-1}(0,t) - \Psi_1(0,t)\right)\,,\\
\cEf{1&-1}{0&0}{x}{\vec a} = \frac{1}{2}\log^2 x + \int_0^xdt_1\,\Psi_1(0,t_1)\int_0^{t_1}dt_2\,\left(\Psi_{-1}(0,t_2) - \Psi_1(0,t_2)\right)\,,\\
\cEf{-1&1}{0&0}{x}{\vec a} = \frac{1}{2}\log^2 x + \int_0^xdt_1\,\Psi_1(0,t_1)\int_0^{t_1}dt_2\,\left(\Psi_{-1}(0,t_2) - \Psi_1(0,t_2)\right)\,,\\
\eeq
The form of the regulated eMPLs seems rather ad hoc. The form is in fact dictated by requiring the  following natural properties:
\begin{enumerate}
\item The regularisation of eMPLs is consistent with the regularisation of ordinary MPLs, i.e., eq.~\eqref{eq:cE4_to_G} still holds after regularisation.
\item The regularisation preserves the shuffle algebra structure, i.e., 

%\paragraph{Functional relations of uniform weight.} We observe empirically in all case that the weight is preserved by relations relating eMPLs with different arguments. For example, consider the following function
%\beq\label{eq:kite_log}
%f(x) = \log\frac{v[\mu_1+(1-\mu_3)(1-v)]+\mu_2(1-v) -(1+\mu_3)y}{v[\mu_1+(1-\mu_3)(1-v)]+\mu_2(1-v) +(1+\mu_3)y}\,.
%\eeq
%The variable $y$ is not an independent variable, but it is constrained by the quartic polynomial equation
%\beq\label{eq:kite_curve}
%y^2 = x^4 + c_3\,x^3+c_2\,x^2+c_1\,x+c_0 = (x-a_1)(x-a_2)(x-a_3)(x-a_4)\,.
%\eeq
%The coefficients appearing inside the quartic polynomial are
%\beq\bsp
%c_3&\,=\frac{2 \left(-\mu _3^2+\mu _1 \mu _3-\mu _2 \mu _3+2 \mu _3+\mu _1-\mu _2-1\right)}{\left(\mu _3-1\right)^2}\,\\
%c_2 &\, =\frac{\mu _1^2-2 \mu _2 \mu _1-2 \mu _3 \mu _1-2 \mu _1+\mu _2^2+\mu _3^2+4 \mu _2+4 \mu _2 \mu _3-2 \mu _3+1}{\left(\mu _3-1\right)^2}\,,\\
%c_1&\,=-\frac{2 \mu _2 \left(-\mu _1+\mu _2+\mu _3+1\right)}{\left(\mu _3-1\right)^2}\,,\\
%c_0 &\,= \frac{\mu _2^2}{\left(\mu _3-1\right)^2}\,.
%\esp\eeq
%The roots $a_i$ of the quartic polynomial are complicated algebraic functions whose explicit form is irrelevant for the following. The logarithm in eq.~\eqref{eq:kite_log} appears in the computation of the two-loop kite integral with three different masses~\cite{ourkite}, with $\mu_i=m_i^2/p^2>1$ and $x$ is a Feynman parameter that still needs to be integrated over the range $[0,1]$. In order to perform the integral over $x$, it is useful to cast this logarithm in the form of an integral where $x$ only appears as the upper integration limit. Since eq.~\eqref{eq:kite_curve} defines an elliptic curve, it is easy to see that such an integral representation will involve eMPLs. Indeed, we find,
%\beq\bsp\label{eq:kite_example}
%f(x) &\,= \log\mu_2 + \cEf{-1}{\infty}{x}{\vec{a}} - \cEf{-1}{\frac{\mu_2}{\mu_2-\mu_1}}{x}{\vec{a}} -\cEf{-1}{0}{x}{\vec{a}}\\
%&\,-\cEf{-1}{1}{x}{\vec{a}}-4\pi i\, \cEf{0}{0}{x}{\vec{a}}\,.
%\esp\eeq
%We see that every term in the right-hand side has weight one, just like the logarithm in eq.~\eqref{eq:kite_log}. We stress that it is crucial that the weight is not identified with the number of integrations, because otherwise the last term in eq.~\eqref{eq:kite_example} would not have weight one. We have derived a large variety of identities of this type up to weight three, and in all cases we observe that the weight is conserved. We therefore conjecture that this observation holds in general, and extends the corresponding property for ordinary MPLs.

%\paragraph{Ordinary MPLs with arguments that are rational functions on an elliptic curve.} Consider the function $F(x) = G(R_1(x,y),\ldots,R_n(x,y);R_{n+1}(x,y))$, where the $R_i$ are rational functions with $y^2=P_4(x)$. In ref.~\cite{Broedel:2017kkb} it was shown that every function of this type can be written in terms of the (non-pure) eMPLs $\textrm{E}_4$. The function $F$, however, is a pure function in the traditional sense. If our extension of pure functions to the elliptic case is consistent, we must always be able to write $F$ as a pure combination of $\cE_4$ functions. In the following we argue that this is indeed always possible. 
%
%First, from eq.~\eqref{eq:MPL_tot_diff} we see that the claim follows recursively if we manage to write the logarithmic one-forms $d\log(P(x)+ y\, Q(x))$, where $P$ and $Q$ are polynomials, in terms of the one-forms $dx\,\Psi_{\pm n}(c,x,\vec a)$ which define the iterated integrals $\cE_4$. We have
%\beq\bsp
%d\log(P(x)+ y Q(x)) &\,= \frac{1}{2} d\log(P(x)^2-y^2Q(x)^2) + \frac{1}{2}d\log\left(\frac{P(x)+y\,Q(x)}{P(x)-y\,Q(x)}\right) \\
%&\,=\frac{1}{2}d\log\left(\frac{P(x)+y\,Q(x)}{P(x)-y\,Q(x)}\right)  + \frac{1}{2}\sum_i d\log(x-x_i) \\
%&\,=\frac{1}{2}d\log\left(\frac{P(x)+y\,Q(x)}{P(x)-y\,Q(x)}\right)  + \frac{1}{2}\sum_i dx\,\Psi_1(x_i,x,\vec a)\,,
%\esp\eeq 
%where the sum runs over the roots $x_i$ of the polynomial $P(x)^2-y^2Q(x)^2$. The logarithmic one-form in the last line can be written as
%\beq\bsp
%d&\log\left(\frac{P(x)+y\,Q(x)}{P(x)-y\,Q(x)}\right)= \frac{c_4\,dx}{y}\,N(x)\,,
%\esp\eeq
%where $N(x)$ is a rational function of $x$,
%\beq
%\!\!\!\!N(x) = \frac{y^2}{c_4\,(P(x)^2-y^2Q(x)^2)}\left[2P(x)Q'(x) - 2P'(x)Q(x)+P(x)Q(x)\sum_{i=1}^4\frac{1}{x-a_i}\right]\,.
%\eeq
%It is easy to check that the only poles in $N(x)$ come from the vanishing of $P(x)^2-y^2Q(x)^2$. A straightforward computation shows that the residues at these poles are all $\pm1$,
%\beq
%d\log\left(\frac{P(x)+y\,Q(x)}{P(x)-y\,Q(x)}\right) \sim s_i\,\frac{dx}{x-x_i}\,,\qquad s_i\pm 1\,,\qquad x\sim x_i\,.
%\eeq
%Next, let us consider the one-form
%\beq\bsp
%\omega&\,=d\log\left(\frac{P(x)+y\,Q(x)}{P(x)-y\,Q(x)}\right) - \sum_idx\,s_i\,\Psi_{-1}(x_i,x,\vec a)\,.
%\esp\eeq
%We can change coordinates to the coordinate $z\equiv z_x$ on the torus, and using eq.~\eqref{eq:psi_to_g} we find,
%\beq
%\omega = dz\,\Omega(z) = dz\left[\omega_1\,N(\kappa(z,\vec a)) - \sum_{i}s_i\,\left(g^{(1)}(z-z_{x_i},\tau)-g^{(1)}(z+z_{x_i},\tau)\right)\right]\,.
%\eeq
%The function $\Omega(z)$ is meromorphic and double periodic, $\Omega(z+1)=\Omega(z+\tau) = \Omega(z)$, and so it is an elliptic function. By construction, it has no poles, and one can show that every elliptic function without poles is constant. While we do not have a derivation of the value of that constant, we have computed it numerically for several hundreds of polynomials $P$ and $Q$ of small degree and random values for the coefficients. In all cases we find that the value of the constant $\Omega(z)$ is zero, and we therefore conjecture this to hold in general. Based on this conjecture, we conclude that
%\beq\bsp\label{eq:pure_dlog}
%d\log(P(x)+ y Q(x)) &\,= \frac{1}{2}\sum_i dx\,\left[\Psi_1(x_i,x,\vec a)+s_i\,\Psi_{-1}(x_i,x,\vec a)\right]\,,
%\esp\eeq 
%which finishes the argument. 
%We then conclude that $G(R_1(x,y),\ldots,R_n(x,y);R_{n+1}(x,y))$ can always be written as a $\mathbb{Q}$-linear combination of  $\cEf{n_1 & \ldots & n_k}{c_1 & \ldots& c_k}{x}{\vec{a}}$, with $n_i=\pm 1$.
%
%
%
























